Evaluating Self-Supervised Learning for Molecular Graph Embeddings

Graph Self-Supervised Learning (GSSL) provides a robust pathway for acquiring embeddings without expert labelling, a capability that carries profound implications for molecular graphs due to the staggering number of potential molecules and the high cost of obtaining labels. However, GSSL methods are designed not for optimisation within a specific domain but rather for transferability across a variety of downstream tasks. This broad applicability complicates their evaluation. Addressing this challenge, we present "Molecular Graph Representation Evaluation" (MOLGRAPHEVAL), generating detailed profiles of molecular graph embeddings with interpretable and diversified attributes. MOLGRAPHEVAL offers a suite of probing tasks grouped into three categories: (i) generic graph, (ii) molecular substructure, and (iii) embedding space properties. By leveraging MOLGRAPHEVAL to benchmark existing GSSL methods against both current downstream datasets and our suite of tasks, we uncover significant inconsistencies between inferences drawn solely from existing datasets and those derived from more nuanced probing. These findings suggest that current evaluation methodologies fail to capture the entirety of the landscape.

==> checklist.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}

%%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNA{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerNA{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}

\item If you ran experiments (e.g. for benchmarks)...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerYes{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerYes{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

==> tables/01downstream_large.tex <==
\begin{table}[b!]
\vspace{-1ex}
\caption{
\textbf{Evaluating GSSL methods on molecular property prediction tasks:} For each downstream task, we report the mean (and standard deviation) ROC-AUC of three seeds with scaffold splitting. The best and second best results are marked \textbf{\underline{bold}} and \textbf{bold}, respectively. \revision{We denote the percentage of GSSL that do not outperform \method{Random} (``GSSL Worse'')}. For fair comparison, we also train and report the average scores w/o fine-tuning (Avg/Avg(FT)) on downstream tasks. %\qi{Say more explicitly Avg is w/o FT?}
\vspace{1.2ex}
}
\label{tab:downstream_large}
% \small
\setlength{\tabcolsep}{2.7pt}
\centering
\scalebox{0.85}{
\begin{tabular}{l | c c c c c c c c | c | c}
\toprule
Dataset & BBBP $\uparrow$ & Tox21 $\uparrow$ & ToxCast $\uparrow$ & Sider $\uparrow$ & ClinTox $\uparrow$ & MUV $\uparrow$ & HIV $\uparrow$ & Bace $\uparrow$ & Avg $\uparrow$ & Avg(FT) $\uparrow$\\
\midrule
\# Molecules & 2,039 & 7,831 & 8,575 & 1,427 & 1,478 & 93,087 & 41,127 & 1,513 & -- & -- \\
\# Tasks & 1 & 12 & 617 & 27 & 2 & 17 & 1 & 1 & -- & -- \\
\midrule
\textsc{Random} & 51.9${}_{\pm0.2}$ & 65.6${}_{\pm0.4}$ & 53.3${}_{\pm0.2}$ & 57.6${}_{\pm0.1}$ & 52.2${}_{\pm0.0}$ & \textbf{53.7}${}_{\pm0.4}$ & 67.6${}_{\pm0.4}$ & 69.1${}_{\pm0.2}$ & 58.85 & 67.21 \\
\midrule
\textsc{EdgePred} & 57.9${}_{\pm0.1}$ & 53.2${}_{\pm0.6}$ & 52.9${}_{\pm0.0}$ & 48.6${}_{\pm0.4}$ & 51.5${}_{\pm0.0}$ & \textbf{\underline{53.9}}${}_{\pm0.2}$ & 69.1${}_{\pm0.0}$ & 67.6${}_{\pm0.3}$ & 56.85 & 65.64 \\
\textsc{AttrMask}     & 60.4${}_{\pm0.8}$ & 66.7${}_{\pm0.7}$ & 56.5${}_{\pm0.6}$ & \textbf{60.0}${}_{\pm0.4}$ & 61.4${}_{\pm0.8}$ & 46.2${}_{\pm0.7}$ & 65.4${}_{\pm0.6}$ & \textbf{80.8}${}_{\pm0.4}$ & 62.18 & 70.16 \\
\textsc{GPT-GNN}      & 64.1${}_{\pm0.0}$ & 62.1${}_{\pm0.1}$ & 53.2${}_{\pm0.8}$ & 58.4${}_{\pm0.1}$ & 64.3${}_{\pm0.0}$ & 46.5${}_{\pm0.1}$ & 69.0${}_{\pm0.3}$ & 73.8${}_{\pm0.3}$ & 61.43 & 68.27 \\
\textsc{InfoGraph}    & \textbf{66.3}${}_{\pm0.6}$ & 68.1${}_{\pm0.6}$ & 58.4${}_{\pm0.6}$ & 57.1${}_{\pm0.8}$ & \textbf{\underline{66.3}}${}_{\pm0.6}$ & 44.3${}_{\pm0.6}$ & 70.2${}_{\pm0.6}$ & 64.8${}_{\pm0.8}$ & 61.94 & 70.10 \\
\textsc{Cont.Pred} & 54.6${}_{\pm0.2}$ & 65.0${}_{\pm0.8}$ & 56.5${}_{\pm0.1}$ & 59.8${}_{\pm0.2}$ & 52.1${}_{\pm0.2}$ & 50.6${}_{\pm0.5}$ & 65.3${}_{\pm0.1}$ & 72.7${}_{\pm0.9}$ & 59.58 & \textbf{\underline{70.89}} \\
\textsc{G-Cont.} & 61.2${}_{\pm0.2}$ & \textbf{\underline{69.7}}${}_{\pm2.3}$ & 58.1${}_{\pm0.2}$ & \textbf{\underline{61.7}}${}_{\pm1.9}$ & 70.3${}_{\pm0.2}$ & 44.1${}_{\pm1.6}$ & \textbf{71.0}${}_{\pm0.2}$ & \textbf{\underline{80.9}}${}_{\pm1.9}$ & \textbf{\underline{64.63}} & 69.21 \\
\textsc{G-Motif}      & 66.1${}_{\pm1.0}$ & 65.6${}_{\pm0.7}$ & \textbf{\underline{58.7}}${}_{\pm1.2}$ & 58.7${}_{\pm1.1}$ & \textbf{65.0}${}_{\pm1.0}$ & 39.2${}_{\pm0.7}$ & \textbf{\underline{71.4}}${}_{\pm1.2}$ & 75.9${}_{\pm1.1}$ & 62.59 & 70.14 \\
\textsc{GraphCL}     & 61.6${}_{\pm1.1}$ & 67.5${}_{\pm0.8}$ & \textbf{58.5}${}_{\pm0.9}$ & 57.6${}_{\pm0.8}$ & 74.1${}_{\pm1.1}$ & 44.0${}_{\pm0.8}$ & 67.7${}_{\pm0.9}$ & 73.1${}_{\pm0.8}$ & \textbf{63.00} & \textbf{70.64} \\
\textsc{JOAO}     & 63.8${}_{\pm0.7}$ & 67.6${}_{\pm0.7}$ & 57.1${}_{\pm0.7}$ & 57.1${}_{\pm0.7}$ & 59.2${}_{\pm0.7}$ & 42.9${}_{\pm0.7}$ & 69.4${}_{\pm0.7}$ & 70.8${}_{\pm0.7}$ & 60.99 & 69.57 \\
\textsc{JOAOv2}   & \textbf{\underline{66.4}}${}_{\pm0.9}$ & \textbf{68.2}${}_{\pm0.8}$ & 57.0${}_{\pm0.5}$ & 59.1${}_{\pm0.7}$ & 64.5${}_{\pm0.9}$ & 47.4${}_{\pm0.8}$ & 68.4${}_{\pm0.5}$ & 67.4${}_{\pm0.7}$ & 62.31 & 70.21 \\
\midrule
GSSL Worse    & 10\%      & 20\%      & 10\%      & 30\%      & 20\%      & 90\%      & 20\%      & 30\%      & 10\%  & 10\%  \\
\bottomrule
\end{tabular}}
% \vspace{-2ex}
\end{table}


==> tables/02tabular.tex <==
\begin{table}[b]
\vspace{-1ex}
\caption{\textbf{ROC-AUC scores of classifiers predicting molecular properties (like in \Cref{sec:molecular_prediction})}.\vspace{2ex}}
\label{tab:tabular}
\setlength{\tabcolsep}{4pt}
\centering
\begin{tabular}{ccc|cc}
\toprule
\method{Linear Regression} & \method{Random Forest} & \method{XGBoost} & \method{Random} & \method{GraphCL} \\
\midrule
 59.91 & 61.95 & 62.31 & 58.85 & 63.00 \\
\bottomrule
\end{tabular}
% \vspace{-1ex}
\end{table}


==> tables/03cramerv.tex <==
\begin{wraptable}{r}{0.5\textwidth}
\vspace{2ex}
\centering
\setlength{\tabcolsep}{7pt}
\caption{
Cramér's V between molecular substructure counts and binary properties, averaged over 678 binary property prediction tasks (``Avg, Task'') or eight downstream datasets (``Avg, Data''). We also calculate the Spearman rank correlation ($\rho$) between the performance of recognising substructures and the performance of predicting molecular properties.
\label{tab:cramerv}}
\vspace{-0.5ex}
\begin{tabular}{l|l|ccc}
\toprule
Name & Avg, Task & Avg, Data & $\rho$\\
\midrule
   allylic & 0.1144 & 0.1024 & 0.709 \\
   benzene & 0.1630 & 0.1227 & 0.576 \\
     amide & 0.0881 & 0.1336 & 0.468 \\
     ether & 0.1034 & 0.1083 & 0.552 \\
   halogen & 0.1721 & 0.1086 & 0.515 \\
\bottomrule
\end{tabular}
\vspace{-2ex}
\end{wraptable}

==> tables/03structual_metric.tex <==
\begin{table}[b]
% \vspace{-2ex}
\caption{Benchmarking topological properties. We report the mean square error or the cross entropy on eight datasets. We \textbf{bold} the best and \underline{underline} the worst performance of each metric. We also report the average ranks of each model on these metrics (``R''). \label{tab:probe}}
\vspace{1ex}
\small
\setlength{\tabcolsep}{1.8pt}
\centering
\begin{tabular}{l | c c c | c | c c c | c | c c c c | c }
\toprule
\multirow{2}{*}{Metrics}  & \multicolumn{4}{c|}{Node} & \multicolumn{4}{c|}{Pair} & \multicolumn{5}{c}{Graph}\\
% \midrule
\cmidrule{2-14}
            %  & Degree & Centrality & Cluster & Link & Jaccord & Katz & Diameter & Connectivity & Cycle & Assortativity \\
            & Degree & Cent. & Cluster & R & Link & Jaccord & Katz & R & Diameter & Conn. & Cycle & Assort. & R \\
\midrule
% \textsc{Random}      & \textbf{0.001} & 1.199 & 0.297 & \textbf{1.7} & \textbf{31.05} & 1.879 & \underline{2.828} & 4.7 & \underline{222.6} & \underline{0.226} & \underline{6.351} & \underline{0.158} & \underline{10} \\
\textsc{Random}      & \textbf{0.001} & 1.199 & 0.297 & \textbf{1.7} & \textbf{31.05} & 1.879 & \underline{2.828} & 5 & 222.6 & 0.276 & 9.351 & 0.198 & 10 \\
\midrule
\textsc{EdgePred}     & 0.993 & \underline{1.712} & 0.513 & 9.3 & \underline{71.49} & 2.169 & 2.772 & 9.3 & \underline{250.6} & \underline{0.287} & \underline{19.95} & \underline{0.206} & \underline{11} \\
\method{AttrMask}     & 0.015 & 1.307 & 0.424 & 5 & 32.23 & 2.029 & 2.634 & 4.3 & 164.7 & 0.178 & 6.075 & 0.102 & 3.8 \\
GPT-GNN      & 3.032 & 1.380 & 0.505 & 9 & 41.44 & \underline{2.541} & 2.374 & 8.3 & 178.8 & 0.247 & 9.222 & 0.166 & 8.3 \\
\method{InfoGraph}    & 1.298 & 1.242 & \textbf{0.296} & 4 & 41.15 & 2.273 & 2.238 & 5.7 & \textbf{83.24} & 0.204 & 6.169 & 0.159  & 4.3 \\
\method{Cont.Pred}  & 5.498 & \underline{1.626} & 0.316 & 8 & 37.78 & 2.286 & 2.413 & 7.3 & 183.0 & 0.194 & 8.691 & 0.108  & 5.8 \\
\method{G-Motif}      & 3.085 & 1.372 & \underline{0.531} & \underline{9.7} & 51.83 & 2.363 & 2.758 & \underline{9.7} & 98.21 & 0.268 & 7.333 & 0.182  & 7.5 \\
\method{G-Cont.} & 0.036 & 1.242 & 0.403 & 3.3 & 33.55 & \textbf{1.773} & 2.660 & 4.3 & 113.6 & \textbf{0.170} & \textbf{5.330} & \textbf{0.045}  & \textbf{2.3}\\
\method{GraphCL}      & 0.854 & \textbf{1.110} & 0.461 & 4.7 & 34.97 & 1.863 & \textbf{2.271} & \textbf{3.3} & 89.79 & 0.226 & 6.191 & 0.152  & 5.8 \\
\method{JOAO}         & 0.637 & 1.268 & 0.412 & 5 & 33.67 & 2.084 & 2.307 & 4.7 & 89.38 & 0.214 & 5.960 & 0.142  & 3.5 \\
\method{JOAOv2}       & 0.591 & 1.272 & 0.463 & 6 & 32.81 & 2.054 & 2.340 & 4 & 88.27 & 0.217 & 5.964 & 0.148  & 4.0 \\
\midrule
GSSL Worse  & 100\% & 90\%  & 90\%  & 100\% & 100\% & 80\%  & 0\%  & 50\% & 10\% & 10\% & 10\% & 10\% & 10\% \\
\bottomrule
\end{tabular}
\end{table}


==> tables/04layer.tex <==
\begin{table}[b!]
% \vspace{-2ex}
\caption{Performance on the topological metrics prediction with embeddings extracted from different layers. We report the mean square error or the cross entropy loss (the smaller the better). We \textbf{bold} the best and \underline{underline} the worst performance on node degree (ND) and graph diameter (GD).
\label{tab:layer}}
\vspace{1.2ex}
\setlength{\tabcolsep}{1.3pt}
\centering
\begin{tabular}{l | c c c c c | c c c c c | c c c  c c}
\toprule
 & \multicolumn{5}{c|}{\method{Random}} & \multicolumn{5}{c|}{\method{AttrMask}} & \multicolumn{5}{c}{\method{GraphCL}}\\
\midrule
 & 1 & 2 & 3 & 4 & 5 & 1 & 2 & 3 & 4 & 5 & 1 & 2 & 3 & 4 & 5 \\
\midrule
 ND &  
\underline{0.031} & 0.013 & 0.007 & \textbf{0.001} & \textbf{0.001} & 
\textbf{0.009} & \underline{0.024} & 0.019 & 0.013 & 0.015 & 
\textbf{0.016} & 0.361 & 0.426 & 0.583 & \underline{0.854}\\
 GD &  
184.0 & \underline{236.2} & \textbf{167.4} & 184.0 & 222.5 & 
\underline{198.9} & 181.9 & 184.6 & 171.7 & \textbf{164.7} & 
93.34 & \underline{131.5} & 97.43 & 95.19 & \textbf{89.79}\\
% \midrule
\bottomrule
\end{tabular}
\end{table}

==> tables/05cramerv.tex <==
\begin{table}[b!]
\vspace{-2ex}
\centering
\setlength{\tabcolsep}{10pt}
\caption{Cramér's V between molecular substructure counts and binary properties, averaged over 678 binary property prediction tasks or eight downstream datasets.\label{tab:cramerv}}
\vspace{2ex}
\begin{tabular}{l|ccccc}
\toprule
 & allylic & benzene & amide & ether & halogen \\ \midrule
Cramér's V (task) & 0.1144 & 0.1630 & 0.0881 & 0.1034 & 0.1721 \\
Cramér's V (dataset) & 0.1024 & 0.1227 & 0.1336 & 0.1083 & 0.1086 \\
\bottomrule
\end{tabular}
\vspace{-2ex}
\end{table}

==> tables/065spectrum.tex <==
\begin{wraptable}{r}{0.39\textwidth}
% \vspace{0.9ex}
\vspace{-.7ex}
\caption{Benchmarking the magnitude of the singular values in the spectrum. 
% We provide detailed results in~\Cref{append_sec:subs}.
% \vspace{1ex}
}
\label{tab:spectrum_main}
% \small
\setlength{\tabcolsep}{3.8pt}
\centering
\begin{tabular}{l | c c c }
\toprule
No. Dim        & 1 & 50 & 100 \\
\midrule
\method{Random}       & -2.95 & -14.9 & -17.0 \\\midrule
\method{EdgePred}     & -32.3 & -49.8 & -69.1 \\
\method{AttrMask}     & 1.16  & -10.3 & -12.9 \\
\method{GPT-GNN}      & 2.51  & -8.61 & -10.6 \\
\method{InfoGraph}    & 3.08  & -2.15 & -4.91 \\
\method{Cont.Pred}    & 1.88  & -11.9 & -14.8 \\
\method{G-Motif}      & 4.70  & -0.91 & -4.48 \\
\method{G-Cont.}      & 3.15  & -4.14 & -7.09  \\
\method{GraphCL}      & 3.69  & -4.38 & -7.66  \\
\method{JOAO}         & 3.59  & -4.28 & -7.44 \\
\method{JOAOv2}       & 3.85  & -4.98 & -7.88 \\
\midrule
GSSL smaller          & 10\%  & 10\%  & 10\%  \\
\midrule
Rank Corr.            & 0.809 & 0.755 & 0.755   \\
\bottomrule
\end{tabular}
\vspace{-4ex}
\end{wraptable}

==> tables/06substructure_main.tex <==
\begin{wraptable}{r}{0.6\textwidth}
\vspace{-2.5ex}
\caption{Benchmarking substructure properties. 
% We provide detailed results in~\Cref{append_sec:subs}.
\vspace{-.5ex}
}
\label{tab:substructure_main}
% \small
\setlength{\tabcolsep}{3.6pt}
\centering
\begin{tabular}{l | c c c c c c c c c c c c}
\toprule
                      & allylic & amide & benzene & ether & halogen \\
\midrule
\method{Random}       & 3.516 & 18.948 & 3.964 & 6.071  & 3.652 \\
\midrule
\method{EdgePred}     & \underline{5.854} & \underline{25.126} & \underline{9.804} & \underline{12.838} & \underline{5.214} \\
\method{AttrMask}     & 3.371 & 12.932 & 2.860 & 4.958  & 1.192 \\
\method{GPT-GNN}      & 2.808 & 15.736 & 2.938 & 5.932  & 2.912 \\
\method{InfoGraph}    & 2.577 & 5.535  & 1.959 & 3.657  & 2.819 \\
\method{Cont.Pred}    & 4.386 & 18.251 & 3.583 & 7.045  & 2.908 \\
\method{G-Motif}      & 2.452 & 4.015  & 2.116 & 3.507  & 1.125 \\
\method{G-Cont.}      & 2.196 & 5.938  & 1.926 & \textbf{2.900}  & 0.759 \\
\method{GraphCL}      & \textbf{2.088} & 3.922 & \textbf{1.722} & 3.766  & 0.798 \\
\method{JOAO}         & 2.385 & 4.030  & 1.746 & 3.376  & \textbf{0.694} \\
\method{JOAOv2}       & 2.122 & \textbf{3.865}  & 1.773 & 3.388  & 0.695 \\
\midrule
GSSL Worse             & 20\%  & 10\%  & 10\%  & 20\%  & 10\%  \\
\midrule
Rank Corr.         & 0.709  & 0.576  & 0.468  & 0.552  & 0.515  \\
\bottomrule
\end{tabular}
\vspace{-4ex}
\end{wraptable}


==> tables/07uniformity.tex <==
\begin{table}[t!]
\caption{
\textbf{Evaluating GSSL methods on uniformity}
\vspace{.7ex}
}
\label{tab:uniformity}
\setlength{\tabcolsep}{4pt}
\centering
% \scalebox{0.85}{
\begin{tabular}{l | c c c c c c c c }
\toprule
Dataset & BBBP $\downarrow$ & Tox21 $\downarrow$ & ToxCast $\downarrow$ & Sider $\downarrow$ & ClinTox $\downarrow$ & MUV $\downarrow$ & HIV $\downarrow$ & Bace $\downarrow$\\
\midrule
\textsc{Random}    & -0.001  & -0.002  & -0.002  & -0.002  & -0.001  & -0.001  & -0.001  & -0.000  \\
\midrule
\textsc{EdgePred}  & 0.000   & 0.000   & 0.000   & 0.000   & 0.000   & -0.000  & -0.000  & 0.000  \\
\textsc{AttrMask}  & -0.006  & -0.011  & -0.011  & -0.009  & -0.008  & -0.005  & -0.008  & -0.004 \\
\textsc{GPT-GNN}   & -0.017  & -0.020  & -0.020  & -0.017  & -0.020  & -0.011  & -0.014  & -0.010 \\
\textsc{InfoGraph} & -0.210  & -0.256  & -0.256  & -0.222  & -0.233  & -0.183  & -0.208  & -0.110 \\
\textsc{Cont.Pred} & -0.010  & -0.016  & -0.016  & -0.015  & -0.013  & -0.005  & -0.010  & -0.007 \\
\textsc{G-Cont.}   & -0.012  & -0.015  & -0.015  & -0.013  & -0.013  & -0.010  & -0.013  & -0.006 \\
\textsc{G-Motif}   & -0.023  & -0.023  & -0.024  & -0.023  & -0.023  & -0.021  & -0.023  & -0.020 \\
\textsc{GraphCL}   & -0.091  & -0.118  & -0.117  & -0.093  & -0.099  & -0.082  & -0.092  & -0.062 \\
\textsc{JOAO}      & -0.071  & -0.091  & -0.091  & -0.071  & -0.080  & -0.063  & -0.069  & -0.047 \\
\textsc{JOAOv2}    & -0.053  & -0.067  & -0.066  & -0.053  & -0.062  & -0.045  & -0.047  & -0.033 \\
\midrule
GSSL Worse         & 10\%    &  10\%   & 10\%& 10\%& 10\%& 10\%& 10\%& 10\%\\
\midrule
Rank Corr.         & -0.509	 & -0.436  & -0.436	& -0.436 & -0.489 & -0.531 & -0.509 & -0.408 \\
\bottomrule
\end{tabular}
% }
% \vspace{-2ex}
\end{table}


==> tables/08reinit.tex <==
\begin{table}[H]
\caption{Probe measures after re-initialising parts of weights of the pre-trained GNNs. We \textbf{bold} the best and \underline{underline} the worst performance of each (pre-trained) embeddings on each structural metric. The digits in the ``Re-Init'' row represent the index/location of re-initialised GIN convolutional layers.
\label{tab:reinit}}
\vspace{-1ex}
\setlength{\tabcolsep}{1.9pt}
\centering
\begin{tabular}{l | c c c c c c c | c c c cc  c c}
\toprule
& \multicolumn{7}{c|}{\method{AttrMask}} & \multicolumn{7}{c}{\method{GraphCL}}\\
\midrule
& None & Embed & 1 & 2 & 3 & 4 & 5 & None & Embed & 1 & 2 & 3 & 4 & 5 \\
\midrule
ND  & 
\textbf{0.015} & \underline{0.263} & 0.062 & 0.076 & 0.021 & 0.063 & 0.041 & 
\textbf{0.854} & 1.429 & \underline{1.439} & 1.086 & 1.406 & 1.111 & 1.399 \\
GD & 
\textbf{164.7} & 178.4 & 188.5 & 184.6 & 191.1 & 225.1 & \underline{229.7} &  
\textbf{89.79} & 90.14 & 102.6 & 111.5 & 136.5 & 139.5 & \underline{163.9} \\
\bottomrule
\end{tabular}
\end{table}

==> tables/aggregation.tex <==
\begin{wraptable}{r}{0.5\textwidth}
\vspace{-3ex}
\caption{
Probe performance with different aggregation choices in the message passing. The 'Sum' aggregation is the default setting.
\vspace{-1ex}
}
\label{tab:msgpassing}
\setlength{\tabcolsep}{4pt}
\centering
\begin{tabular}{l|l|ccc}
\toprule
Metric & Aggr & Random & AttrMask &  GraphCL \\
\midrule
         & Max  & 31.69  & 12.87 & 12.36 \\
Degree   & Sum  & 0.002  & 0.123 & 0.681 \\
         & Mean & 0.003  & 0.064 & 1.381 \\
\midrule
         & Max  & 156.2  & 181.1 & 87.93 \\
Diameter & Sum  & 218.7  & 162.0 & 88.44 \\
         & Mean & 208.2  & 287.2 & 117.2 \\
\bottomrule
\end{tabular}
\end{wraptable}


==> tables/substructure_1.tex <==
\begin{table}[H]
\caption{
Substructure Detection, MSE Loss, Part I
\vspace{2ex}
}
\small
\label{tab:substructure_app}
\setlength{\tabcolsep}{2pt}
\centering
\begin{tabular}{l | c c c c c c c c c c c c}
\toprule
Pre-training & allylic & amide & amidine & Azo & benzene & epoxide & ether & furan & guanido & halogen & imidazole & imide \\
\midrule
--           & 3.516 & 18.948 & 0.370 & 0.216 & 3.964 & 0.146 & 6.071  & 0.536 & 0.217 & 3.652 & 0.531 & 0.417 \\
\midrule
\method{EdgePred}     & 5.854 & 25.126 & 0.417 & 0.251 & 9.804 & 0.154 & 12.838 & 0.705 & 0.249 & 5.214 & 0.597 & 0.578 \\
\method{AttrMask}     & 3.371 & 12.932 & 0.364 & 0.174 & 2.860 & 0.123 & 4.958  & 0.242 & 0.213 & 1.192 & 0.459 & 0.319 \\
\method{GPT-GNN}      & 2.808 & 15.736 & 0.360 & 0.156 & 2.938 & 0.141 & 5.932  & 0.407 & 0.220 & 2.912 & 0.483 & 0.474 \\
\method{InfoGraph}    & 2.577 & 5.535  & 0.327 & 0.143 & 1.959 & 0.116 & 3.657  & 0.116 & 0.207 & 2.819 & 0.302 & 0.326 \\
\method{Cont.Pred}  & 4.386 & 18.251 & 0.356 & 0.198 & 3.583 & 0.137 & 7.045  & 0.507 & 0.203 & 2.908 & 0.520 & 0.488 \\
\method{G-Motif}      & 2.452 & 4.015  & 0.194 & 0.082 & 2.116 & 0.134 & 3.507  & 0.068 & 0.115 & 1.125 & 0.348 & 0.150 \\
\method{G-Cont.} & 2.196 & 5.938  & 0.172 & 0.067 & 1.926 & 0.114 & 2.900  & 0.084 & 0.121 & 0.759 & 0.249 & 0.160 \\
\method{GraphCL}      & 2.088 & 3.922  & 0.262 & 0.124 & 1.722 & 0.127 & 3.766  & 0.074 & 0.167 & 0.798 & 0.274 & 0.192 \\
\method{JOAO}         & 2.385 & 4.030  & 0.280 & 0.113 & 1.746 & 0.115 & 3.376  & 0.061 & 0.168 & 0.694 & 0.237 & 0.192 \\
\method{JOAOv2}       & 2.122 & 3.865  & 0.262 & 0.112 & 1.773 & 0.123 & 3.388  & 0.068 & 0.125 & 0.695 & 0.244 & 0.197 \\
\midrule
SSL Worse    & 20\%  & 10\%   & 10\%  & 10\%  & 10\%  & 10\%  & 20\%   & 10\%  & 20\%  & 10\%  & 10\%  & 20\%  \\
\bottomrule
\end{tabular}
% \vspace{-2ex}
\end{table}


==> tables/substructure_2.tex <==
\begin{table}[H]
\caption{
Substructure Detection, MSE Loss, Part II
\vspace{2ex}
}
\label{tab:substructure_mse2}
\small
\setlength{\tabcolsep}{1.6pt}
\centering
\begin{tabular}{l | c c c c c c c c c c c}
\toprule
Pre-training & lactam & morpholine & NO & oxazole & piperdine & piperzine & pyridine & tetrazole & thiazole & thiophene & urea \\
\midrule
--           & 0.049 & 0.439 & 0.214 & 0.121 & 1.094 & 0.410 & 1.528 & 0.141 & 0.402 & 0.550 & 0.458 \\
\midrule
\method{EdgePred}     & 0.055 & 0.547 & 0.218 & 0.126 & 1.332 & 0.592 & 1.674 & 0.195 & 0.470 & 0.782 & 0.782 \\
\method{AttrMask}     & 0.043 & 0.196 & 0.212 & 0.107 & 0.917 & 0.250 & 1.111 & 0.089 & 0.339 & 0.313 & 0.222 \\
\method{GPT-GNN}     & 0.041 & 0.195 & 0.232 & 0.098 & 0.878 & 0.293 & 1.416 & 0.137 & 0.382 & 0.515 & 0.443 \\
\method{InfoGraph}    & 0.041 & 0.121 & 0.241 & 0.054 & 0.813 & 0.206 & 0.655 & 0.075 & 0.170 & 0.180 & 0.174 \\
\method{Cont.Pred}  & 0.043 & 0.298 & 0.223 & 0.120 & 1.097 & 0.387 & 1.334 & 0.146 & 0.379 & 0.538 & 0.538 \\
\method{G-Motif}      & 0.048 & 0.153 & 0.212 & 0.031 & 0.768 & 0.219 & 0.670 & 0.034 & 0.081 & 0.092 & 0.092 \\
\method{G-Cont.} & 0.041 & 0.096 & 0.126 & 0.050 & 0.653 & 0.149 & 0.668 & 0.032 & 0.129 & 0.104 & 0.103 \\
\method{GraphCL}      & 0.042 & 0.113 & 0.199 & 0.048 & 0.706 & 0.159 & 0.460 & 0.037 & 0.129 & 0.088 & 0.087 \\
\method{JOAO}         & 0.043 & 0.096 & 0.194 & 0.040 & 0.738 & 0.149 & 0.434 & 0.032 & 0.121 & 0.077 & 0.076 \\
\method{JOAOv2}       & 0.042 & 0.123 & 0.204 & 0.041 & 0.706 & 0.146 & 0.446 & 0.037 & 0.136 & 0.083 & 0.083 \\
\midrule
SSL Worse    & 10\%  & 10\%  & 40\%  & 10\%  & 20\%  & 10\%  & 10\%  & 20\%  & 10\%  & 10\%  & 20\%  \\
\bottomrule
\end{tabular}
% \vspace{-2ex}
\end{table}
